Certifying One-Phase Technology-Assisted Reviews

Technology-assisted review (TAR) workflows based on iterative active learning are widely used in document review applications. Most stopping rules for one-phase TAR workflows lack valid statistical guarantees, which has discouraged their use in some legal contexts. Drawing on the theory of quantile estimation, we provide the first broadly applicable and statistically valid sample-based stopping rules for one-phase TAR. We further show theoretically and empirically that overshooting a recall target, which has been treated as innocuous or desirable in past evaluations of stopping rules, is a major source of excess cost in one-phase TAR workflows. Counterintuitively, incurring a larger sampling cost to reduce excess recall leads to lower total cost in almost all scenarios.

==> 07d-CMH.tex <==

\subsection{The CMH Rule} 

 Callaghan and M\"{u}ller-Hansen \cite{callaghan2020statistical} discuss several hybrid stopping rules, one of which incorporates a novel sample-based stopping criterion. Like SPET rules, the rule straddles the line between interventional and standoff rules.  Also like SPET rules, the rule conducts a series of statistical tests with no adjustment for multiple tests. This would normally lead to sequential bias, but the tests have an unusual dependence structure. While Callaghan and M\"{u}ller-Hansen provide no proof that their rule is valid, they find empirically that it actually exceeds its targeted recall and confidence level, suggesting that further analysis is of interest.    
 









    

    














==> 07e-coda.tex <==



\subsection{Coda}


 
Our perhaps surprising conclusion is that all these sample-based stopping rules either fail to meet their stated statistical criteria or incur extreme cost risk. In the next section we show how the QBCB rule allows  QBCB rule.  The open question that remains then is where the appropriate tradeoff lies between the cost of larger samples and the reduction in review cost that those larger samples provide.  We explore this empirically in the remainder of the paper.  

